Precision measurement of the index of refraction of deep glacial ice at radio frequencies at Summit Station, Greenland

Glacial ice is used as a target material for the detection of ultra-high energy neutrinos, by measuring the radio signals that are emitted when those neutrinos interact in the ice. Thanks to the large attenuation length at radio frequencies, these signals can be detected over distances of several kilometers. One experiment taking advantage of this is the Radio Neutrino Observatory Greenland (RNO-G), currently under construction at Summit Station, near the apex of the Greenland ice sheet. These experiments require a thorough understanding of the dielectric properties of ice at radio frequencies. Towards this goal, calibration campaigns have been undertaken at Summit, during which we recorded radio reflections off internal layers in the ice sheet. Using data from the nearby GISP2 and GRIP ice cores, we show that these reflectors can be associated with features in the ice conductivity profiles; we use this connection to determine the index of refraction of the bulk ice as n=1.778 +/- 0.006.

==> author_list.tex <==
% J Glaciology list for RNO-G Collaboration

\author[Aguilar and others]{
  J.~A.~Aguilar$^{1}$,
  P.~Allison$^{2}$,
  D.~Besson$^{3}$,
  A.~Bishop$^{4}$,
  O.~Botner$^{5}$,
  S.~Bouma$^{6}$,
  S.~Buitink$^{7}$,
  M.~Cataldo$^{6}$,
  B.~A.~Clark$^{8}$,
  K.~Couberly$^{3}$,
  Z.~Curtis-Ginsberg$^{9}$,
  P.~Dasgupta$^{1}$,
  S.~de~Kockere$^{10}$,
  K.~D.~de~Vries$^{10}$,
  C.~Deaconu$^{9}$,
  M.~A.~DuVernois$^{4}$,
  A.~Eimer$^{6}$,
  C.~Glaser$^{5}$,
  A.~Hallgren$^{5}$,
  S.~Hallmann$^{11}$,
  J.~C.~Hanson$^{12}$,
  B.~Hendricks$^{13}$,
  J.~Henrichs$^{11,6}$,
  N.~Heyer$^{5}$,
  C.~Hornhuber$^{3}$,
  K.~Hughes$^{9}$,
  T.~Karg$^{11}$,
  A.~Karle$^{4}$,
  J.~L.~Kelley$^{4}$,
  M.~Korntheuer$^{1}$,
  M.~Kowalski$^{11,14}$,
  I.~Kravchenko$^{15}$,
  R.~Krebs$^{13}$,
  R.~Lahmann$^{6}$,
  U.~Latif$^{10}$,
  J.~Mammo$^{15}$,
  M.~J.~Marsee$^{16}$,
  Z.~S.~Meyers$^{11,6}$,
  K.~Michaels$^{9}$,
  K.~Mulrey$^{17}$,
  M.~Muzio$^{13}$,
  A.~Nelles$^{11,6}$,
  A.~Novikov$^{18}$,
  A.~Nozdrina$^{3}$,
  E.~Oberla$^{9}$,
  B.~Oeyen$^{19}$,
  I.~Plaisier$^{6,11}$,
  N.~Punsuebsay$^{18}$,
  L.~Pyras$^{11,6}$,
  D.~Ryckbosch$^{19}$,
  O.~Scholten$^{10,20}$,
  D.~Seckel$^{18}$,
  M.~F.~H.~Seikh$^{3}$,
  D.~Smith$^{9}$,
  J.~Stoffels$^{10}$,
  D.~Southall$^{9}$,
  K.~Terveer$^{6}$,
  S.~Toscano$^{1}$,
  D.~Tosi$^{4}$,
  D.~J.~Van~Den~Broeck$^{10,7}$,
  N.~van~Eijndhoven$^{10}$,
  A.~G.~Vieregg$^{9}$,
  J.~Z.~Vischer$^{6}$,
  C.~Welling$^{9}$,
  D.~R.~Williams$^{16}$,
  S.~Wissel$^{13}$,
  R.~Young$^{3}$,
  A.~Zink$^{6}$
}
\affiliation{
 $^{1}$Universit\'e Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium,\\
 $^{2}$Dept.\ of Physics, Center for Cosmology and AstroParticle Physics, Ohio State University, Columbus, OH 43210, USA,\\
 $^{3}$University of Kansas, Dept.\ of Physics and Astronomy, Lawrence, KS 66045, USA,\\
 $^{4}$Wisconsin IceCube Particle Astrophysics Center (WIPAC) and Dept.\ of Physics, University of Wisconsin-Madison, Madison, WI 53703,  USA,\\
 $^{5}$Uppsala University, Dept.\ of Physics and Astronomy, Uppsala, SE-752 37, Sweden,\\
 $^{6}$Erlangen Center for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, 91058 Erlangen, Germany,\\
 $^{7}$Vrije Universiteit Brussel, Astrophysical Institute, Pleinlaan 2, 1050 Brussels, Belgium,\\
 $^{8}$Dept.\ of Physics and Astronomy, Michigan State University, East Lansing MI 48824, USA,\\
 $^{9}$Dept.\ of Physics, Enrico Fermi Inst., Kavli Inst.\ for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA,\\
 $^{10}$Vrije Universiteit Brussel, Dienst ELEM, B-1050 Brussels, Belgium,\\
 $^{11}$Deutsches Elektronen-Synchrotron DESY, Platanenallee 6, 15738 Zeuthen, Germany,\\
 $^{12}$Whittier College, Whittier, CA 90602, USA,\\
 $^{13}$Dept.\ of Physics, Dept.\ of Astronomy \& Astrophysics, Penn State University, University Park, PA 16801, USA,\\
 $^{14}$Institut für Physik, Humboldt-Universit\"at zu Berlin, 12489 Berlin, Germany,\\
 $^{15}$Dept.\ of Physics and Astronomy, Univ.\ of Nebraska-Lincoln, NE, 68588, USA,\\
 $^{16}$Dept.\ of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA,\\
 $^{17}$Dept.\ of Astrophysics/IMAPP, Radboud University, PO Box 9010, 6500 GL, The Netherlands,\\
 $^{18}$Dept.\ of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA,\\
 $^{19}$Ghent University, Dept.\ of Physics and Astronomy, B-9000 Gent, Belgium,\\
 $^{20}$Kapteyn Institute, University of Groningen, Groningen, The Netherlands
}

